Cocktail: Leveraging Ensemble Learning for Optimized Model Serving in Public Cloud

With a growing demand for adopting ML models for a varietyof application services, it is vital that the frameworks servingthese models are capable of delivering highly accurate predic-tions with minimal latency along with reduced deploymentcosts in a public cloud environment. Despite high latency,prior works in this domain are crucially limited by the accu-racy offered by individual models. Intuitively, model ensem-bling can address the accuracy gap by intelligently combiningdifferent models in parallel. However, selecting the appro-priate models dynamically at runtime to meet the desiredaccuracy with low latency at minimal deployment cost is anontrivial problem. Towards this, we proposeCocktail, a costeffective ensembling-based model serving framework.Cock-tailcomprises of two key components: (i) a dynamic modelselection framework, which reduces the number of modelsin the ensemble, while satisfying the accuracy and latencyrequirements; (ii) an adaptive resource management (RM)framework that employs a distributed proactive autoscalingpolicy combined with importance sampling, to efficiently allo-cate resources for the models. The RM framework leveragestransient virtual machine (VM) instances to reduce the de-ployment cost in a public cloud. A prototype implementationofCocktailon the AWS EC2 platform and exhaustive evalua-tions using a variety of workloads demonstrate thatCocktailcan reduce deployment cost by 1.45x, while providing 2xreduction in latency and satisfying the target accuracy for upto 96% of the requests, when compared to state-of-the-artmodel-serving frameworks.

==> 7-related.tex <==
%%%%%

\textbf{Model-serving in Cloud}: The most relevant prior works to \emph{Cocktail} are InFaas~\cite{infaas} and Clipper~\cite{clipper}, which have been extensively discussed and compared to in Section~\ref{sec:results}. %To summarize: (i) InFaas is limited to single model selection and thus suffers from higher latencies to reach higher accuracy. (ii) Clipper model selection policies are static and hence consume more resources compared to \emph{Cocktail}. In addition the ensemble weight selection policies are complex not scalable for large number of models. 
{\color{blue} Recently FrugalML~\cite{Chen2020FrugalML} was proposed to cost-effectively choose from commercial MLaaS APIs for classification tasks. While striking a few similarities with \emph{Cocktail} it is practically limited to classifications with very few classes and does not address resource provisioning challenges.} Mark~\cite{mark} proposed SLO and cost aware resource procurement policies for model-serving. Although our heterogeneous instance procurement policy strikes some similarities with MArk, it is significantly different because we consider ensemble models. Also, the idea to offload requests to burstable instances for cost-savings can be adapted in \emph{Cocktail}. Rafiki~\cite{rafiki} considers small model sets and scales up and down the ensemble size by trading off accuracy to match throughput demands. However, \emph{Cocktail's} resource management is more adaptive to changing request loads and does not drop accuracy. Pretzel~\cite{pretzel} and Inferline~\cite{inferline} are built on top of Clipper to optimize the prediction pipeline and cost due to load variations, respectively. Many prior  works~\cite{velox,laser,clockwork,swift} have extensively tried to reduce model latency by reducing overheads due to shared resources and hardware interference. We believe the policies proposed in this paper can be complementary and beneficial to these prior works towards reducing the cost and resource footprint of ensembling. There are mainstream commercial systems which automate model-serving like TF-Serving~\cite{serving}, SageMaker~\cite{sagemaker}, AzureML~\cite{azureML}, Deep-Studio~\cite{deepstudio} etc. Unlike \emph{Cocktail}, they do not optimize model ensembling to cost-effectively meet SLO constraints.\\
\begin{table}
\footnotesize
\begin{center}
\resizebox{0.45\textwidth}{!}{%
 \begin{tabular}{||c | c | c | c |c | c | c |c||} 
 \hline
 \textbf{Features} & \begin{turn}{90}Clipper \cite{clipper}\end{turn} &
  \begin{turn}{90}Rafiki\cite{rafiki}\end{turn} &
  \begin{turn}{90}Infaas \cite{infaas}\end{turn} & \begin{turn}{90}Mark \cite{mark}\end{turn} &
 \begin{turn}{90}Sagemaker\cite{sagemaker}\end{turn} &
 \begin{turn}{90}Swayam \cite{swayam}\end{turn}& \begin{turn}{90}\emph{Cocktail} \end{turn} \\
%  \hline
%   \textbf{Cluster Level integration } & \xmark & \xmark & \xmark & \xmark & \xmark & {\cmark} \\  
 \hline
 \textbf{Predictive Scaling} & \xmark & \xmark &  \xmark & \cmark & \xmark & \cmark & \cmark \\  
%  \hline
%  \textbf{QoS Prediction} & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark \\
 \hline
  \textbf{SLO Guarantees} & \cmark & \xmark &  \cmark & \cmark & \xmark & \cmark & \cmark \\
 \hline
  \textbf{Cost Effective} & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \cmark \\
   \hline
   \textbf{Ensembling} & \cmark & \cmark & \xmark & \xmark &\cmark & \xmark & \cmark \\
   \hline
%  \textbf{Utilization Improvement} & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
 \textbf{Heterogeneous Instances} & \xmark & \cmark &  \cmark & \cmark & \cmark &\xmark & \cmark \\
  \hline
 \textbf{Dynamic ensemble selection} & \xmark & \xmark & \xmark & \xmark &\xmark & \xmark & \cmark \\
   \hline
\textbf{Model abstraction} & \cmark & \cmark & \cmark & \xmark &\xmark & \xmark & \cmark \\
%  \textbf{Utilization Improvement} & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark \\
\hline

\end{tabular}}
\end{center}
% \vspace{-1mm}
\caption{{\color{black}Comparing the features of \emph{\emph{Cocktail}} with other state-of-the-art frameworks.}}
  \label{tbl:related}
\end{table}
%\textbf{Model Ensembling} \\
\textbf{Autoscaling in Public Cloud}: There are several research works that optimize for the resource provisioning cost in the public cloud. These works broadly fall into two categories: (i) tuning the autoscaling policy based on changing needs (e.g., Spot,  On-Demand)~\cite{swayam,tributary,proteus,stratus,Wang:2017:UBI:3107080.3084448,burscale,exosphere}, (ii) predicting peak loads and offering proactive provisioning based autoscaling policy~\cite{swayam,mark,10.5555/2748143.2748357,spotcheck,tributary}. \emph{Cocktail} uses similar load prediction models and auto-scales VMs in a distributed fashion with respect to model ensembling. Swayam~\cite{swayam} is relatively similar to our work in  that it handles container provisioning along with load-balancing, specifically catered for single model inferences. \emph{Cocktail's} autoscaling policy strikes parallels with Swayam's distributed autoscaling policy;  however, we further incorporate novel importance sampling techniques to reduce over-provisioning for under-used models. Table~\ref{tbl:related} provides a comprehensive comparison of \emph{Cocktail} with the above mentioned related works across key dimensions.  

%%%%%



==> 8-discussion.tex <==
% \noindent{\textbf{Applicability to other applications:}}  Our model selection policies can be adopted to other domains with minimal development efforts. Also, the class-based weighted majority voting technique can be transformed depending on the application. For instance, in topic modelling recommender systems, the weights can be assigned to unique topic categories. %We plan do this as a part of future work. \\ 

% \textbf{Cloud Platform}: Although we evaluate \emph{Cocktail} using AWS, it can be extended to other major cloud platforms like Azure~\cite{azure} and Google-cloud~\cite{google} because they also offer transient instances.\\ %Note that, private cloud environment can greatly benefit from our model-selection and autoscaling polices  especially in terms of resource consumption and operating costs.\\
% \textbf{Instance Failures}: For applications which cannot tolerate even 0.5\% loss in accuracy, we can potentially use burstable instances as backup to offload the queries of failed transient VMs. This will incurs increased deployment costs compared to spot-instance only deployment. In case of smaller ensembles where accuracy drops will be high due to failures,  we can employ a hybrid design where spot+burstables can be used for smaller ensembles and only spot for large ensembles. 

% methodology of a more efficient policy for the reinforcement learning-based system. Specifically, we would like feedback for the PPO policy -- whether it would be well-suited for the problem we consider and also its applicability at scale. \\ 
% \textbf{Limitations:}  In our characterization studies, we did not include spot and burstable instances for VMs. We plan to consider them as well to develop a holistic system with all types of resource offerings from public cloud.\\ 
% \textbf{Open Problems:} We believe the problem discussed in this work can be addressed from several other dimensions. One promising way to look into the problem is to combine the DNN optimization techniques, e.g., model approximation, reduced precision network, ensemble learning, federated learning, etc., with our approach to deliver the most efficient solutions to the users with respect to cost and latency without (or minimally) compromising accuracy. For instance, with reduced precision activations, we can significantly lower the latency, and hence the cost, with a minimal dip in accuracy (approximately 2\% to 3\%). One more such example could include an ensemble learning approach, where the results from many low-cost and low-latency models with relatively lower accuracy could be aggregated together to give much higher accuracy.  In such scenarios, \emph{spot instances} can be helpful in lowering the cost. Furthermore, newer paradigms such as federated learning can help us efficiently and in a parallel fashion learn the query patterns from different users and help us building a more efficient scheduling policy. In a nutshell, we would like to have a holistic view of all public cloud offerings to build an efficient framework to offer  extremely intelligent, adaptive, yet low latency and low-cost solutions. 

%For instance, we do not account for approximate models (ML models) in our study. Model approximation can further reduce response latency without sacrificing accuracy for several applications. Incorporating them into our system would result in additional cost-savings. Similarly, there are different ways to handle inference queries in federated learning domain. For instance,  multiple inferences queries are executed in parallel and the prediction results can be aggregated together for better accuracy. If there are similar inference queries, and in-case one of them fails, the prediction results can still be inferred from other queries. Spot instances could be well suited to execute these type of inferences which can drastically reduce cost without compromising accuracy. 
